Securing Mobile IoT with Unmanned Aerial Systems

The Internet of Things (IoT) will soon be omnipresent and billions of sensors and actuators will support our industries and well-being. IoT devices are embedded systems that are connected using wireless technology for most of the cases. The availability of the wireless network serving the IoT, the privacy, integrity, and trustworthiness of the data are of critical importance, since IoT will drive businesses and personal decisions. This paper proposes a new approach in the wireless security domain that leverages advanced wireless technology and the emergence of the unmanned aerial system or vehicle (UAS or UAV). We consider the problem of eavesdropping and analyze how UAVs can aid in reducing, or overcoming this threat in the mobile IoT context. The results show that huge improvements in terms of channel secrecy rate can be achieved when UAVs assist base stations for relaying the information to the desired IoT nodes. Our approach is technology agnostic and can be expanded to address other communications security aspects.

==> include/background.tex <==
%%II.	C-V2X RESOURCES AND COMMUNICATIONS PROCEDURES

C-V2X uses the sidelink (SL) for sending and receiving mes-sages between a vehicular UE and an eNB (Mode 3) or among vehicular UEs (Mode 4). The former uses the LTE-Uu interface, whereas the latter uses the new PC5 interface, the direct link between two vehicular UEs. The maximum allowed latency ranges between 20 and 100 ms, depending on the application.
A.	Resources
Sidelink resources are shared with the LTE uplink (UL). C-V2X allows channel bandwidths of 10 and 20 MHz. A channel is further divided into subchannels in the frequency domain and subframes in the time domain. Each subchannel consists of sev-eral resource blocks (RBs). An RB is defined as 12 subcarriers by 1 slot, or 180 kHz by 0.5 ms to be consistent with the LTE UL or downlink (DL) operation. The number of RBs per sub-channel is configurable. 
Maintaining LTE’s transmission time interval (TTI) of 1 ms, the 1 ms subframe constitutes the time granularity of C-V2X messages and is the basis for message scheduling. As with LTE, RBs are thus scheduled in pairs.
The vehicular UE data is carried over the Physical SL Shared Channel (PSSCH), which is transmitted along with the Physical SL Control Channel (PSCCH) that carries the SL control infor-mation (SCI). Two resource configurations are possible: In the adjacent configuration (Fig. 1a), the control and data channels are transmitted in adjacent RBs, occupying one or several sub-channels. The SCI is transmitted in the first two RBs in the reserved subframe—four in total—followed by the data. In the nonadjacent configuration, two separate resource pools are con-figured for the PSCCH and PSSCH (Fig. 1b).
B.	Sidelink Control Information 
SCI Format 1 is introduced in 3GPP R14 for C-V2X, whereas SCI Format 0 remains from R12 for D2D. The SCI is transmitted over the PSCCH and carries the information related to the transmission of data over the PSSCH. SCI Format 1 in-forms the receiving vehicular UEs about the resource reservation interval, the frequency location of initial transmission and re-transmission, the time gap between initial transmission and re-transmission, and the modulation and coding scheme of the PSSCH data.
C.	Physical Layer
As for the LTE UL, the C-V2X channel access is singe-carrier frequency division multiple access (SC-FDMA). The con-trol information is QPSK modulated; QPSK or 16-QAM is used for the data. Only normal cyclic prefix is supported in C-V2X. The last SC-FDMA symbol in each subframe serves as a guard period.
 
Fig. 1.	 Adjacent (a) and nonadjacent (b) PSCCH and PSSCH.
 
Fig. 2.	 Sensing and selection windows for SPS in C-V2X.
C-V2X increases the number of subframes carrying the De-modulation Reference Signal (DMRS) to three per RB for the Physical SL Broadcast Channel (PSBCH) and to four for the PSCCH and PSSCH to account for the high Doppler spread at relative speeds of up to 500 km/h [7].
D.	MAC Layer: Scheduling
In Mode 3, the UEs communicate with the infrastructure or network via eNBs, using the LTE Uu interface. All the control and data signaling is between the C-V2X-enabled UE and the eNB, which also handles the scheduling and centrally controls the access to the radio spectrum. In Mode 4, however, schedul-ing is decentralized and is within the responsibility of the vehic-ular UEs. More precisely, UEs continuously sense the spectrum and select resources for transmission, employing the semi-persistent scheduling (SPS) [8].
SPS was introduced in earlier LTE releases to support ser-vices that require deterministic latency, such as voice. Mode 4 uses it to determine suitable semi-persistent transmission oppor-tunities, i.e. the set of physical subframes and subchannels for regular transmission of messages over a certain time period. 
As illustrated in Fig. 2, vehicular UEs continuously sense the radio frequency (RF) spectrum and use the decoded data over one thousand past subframes to select a set of candidate single-subframe resources within the selection window. A candidate single-subframe resource, which is illustrated as the shaded block in the selection window of Fig. 2, consists of the RBs contained in a subframe and one or more contiguous subchan-nels. The number of required subchannels is a function of the message size. 
The SPS scheduling procedure is as follows: The UE initial-ly considers all resources as candidate resources. A two-step ex-clusion process first excludes those single-subframe resources that have not been monitored. The SPS algorithm then uses the sensing information to discard additional single-subframe re-sources where the reference signal received power (RSRP) is found to be above the established threshold. If more than 20\% of the total resources in the selection window remain, the MAC randomly selects a candidate resource from the 20\% of single-subframe candidate resources with the smallest average SL re-ceived signal strength indicator (S-RSSI). If fewer the 20\% of candidate resources remain in the pool, the threshold is increased by 3 dB and the two-step exclusion process is repeated.
Resources are maintained for a certain number of message transmission intervals. This number is randomly selected in a range that depends on the message rate. Between 5 and 75 transmissions or multiples thereof can be scheduled by the UE with a single SPS invocation [9]. 


==> include/bios.tex <==
\small
\noindent
\textbf{Aly Sabri Abdalla} (asa298@msstate.edu)
is a PhD candidate in the Department of Electrical and Computer Engineering at Mississippi State University. His research interests are on scheduling and congestion control for vehicular ad-hoc and UAV networks.

\vspace{0.2cm}
\noindent
\textbf{Bodong Shang} (bdshang@vt.edu) is currently pursuing Ph.D. degree in the Bradley Department of Electrical and Computer Engineering in Virginia Tech, Blacksburg, USA. His research interests include UAV, Internet of Things, and vehicle-to-everything.

\vspace{0.2cm}
\noindent
\textbf{Vuk Marojevic} (vuk.marojevic@msstate.edu) is an associate professor in electrical and computer engineering at Mississippi State University, Starkville. His research interests include resource management, vehicle-to-everything communications and wireless security %, spectrum sharing, software radios, and wireless network virtualization 
with application to cellular communications, mission-critical networks, and unmanned aircraft systems.

\vspace{0.2cm}
\noindent
\textbf{Lingjia Liu} (ljliu@vt.edu) received his Ph.D. degree in Electrical and Computer Engineering from Texas A\&M University, USA. He is an Associate Professor in the Bradley Department of Electrical and Computer Engineering at Virginia Tech, USA. His research interests include machine learning for wireless communications, 5G and beyond, internet of things.


==> include/platform.tex <==
The proposed security enhancements for integrating UASs into 5G need to be implemented and tested in production like operating environments. On the technology side, this requires 5G systems and configurable radios that act as attackers, relays or enhanced 5G radio or network nodes. On the regulatory side, it needs permissions to radiate in RF spectrum from federal spectrum authorities and licenses holders and adhere to the small UAV operation rules, or special permissions, from federal aviation authorities.

%FIGURE about real AERPAW deployment at MSU
%\hl{Check the figure if you want to add more details(figure commented)}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.495\textwidth]{figures/AERPAW2.jpg}
    \caption{Proposed AERPAW testbed site.}
    \label{fig:aerpaw}
\end{figure}


%Vuk to write text about the PAWR platform and program.

Designed under the Platforms for Advanced Wireless Research program, the \emph{Aerial Platform for Advanced Wireless} (AERPAW) will cover both the technological and regulatory aspects that are needed to operate a 5G testbed with UAVs. It will offer global researchers the opportunity to prototype and experiment advanced wireless technology for emerging UAS applications. Figure~\ref{fig:aerpaw} shows an envisaged testbed site. It will feature experimental base stations and UAVs that communicate via a 5G and software-defined radio (SDR) network. Modern SDRs will be deployed on the fixed towers and lightweight versions will be carried by the UAVs, both implementing advanced wireless protocols. 

Leveraging SDRs, researchers will be able to implement the UAV relays introduced in Section~\ref{sec:results} to improve the secrecy rate and evaluate and extend our simulations results. SDRs will also implement ground or UAV-based RF attacks to test and quantify the vulnerabilities of 5G networks. With the emerging open-source implementations of 5G NR, protocol enhancements can be rapidly prototyped and exhaustively tested in a real setting.

Extensive testing is urgently needed to verify advanced wireless communications and networking systems before, during and after deployment. The first generation of 5G networks are being rolled out at the time of writing and will incrementally improve their security architecture, among others, and support new services and applications. Various potentially harmful 5G attacks are already known today~\cite{jover2019security} and many others will be discovered in the future. Hence, it is critical to have a software-defined community testbed that supports 5G and beyond research and development efforts. AERPAW will allow to collect data in a production like testbed where experiments and results can be reproduced. The sharing of such data will be invaluable for standardization and regulation. %Crowdsourcing, allowing distributed development and testing as well as contributions to specifications 

==> include/procedures.tex <==

%\textbf{To DISCUSS TECHNOLOGY, Opportunities, AND TESTING ALONG WITH A SURVEY of key papers and specifications}


%\subsection{Attacks}

%\subsection{Mitigation}

%One weakness of prior work, e.g.~\cite{zhang19}, is that they outline the attacks, but do not propose robust attack detection and mitigation techniques.


%The 5G specification and provided technology can be utilized to provide more security and robustness for the FANETs nodes and available A2G and UAV-to-UAV links. 3GPP started to give more attention to UAVs and provide more serving services for it in Release 15 of their standard LTE\_Aerial and their initial 5G New Radio (NR)%cite.
%The NR network is designed to be compatible with different 
This section discusses a selected subset of unique procedures for enhancing the security of 5G networks for UAVs and with UAVs. 
Table \ref{tab:my-table2} summarizes the critical security requirements and several promising opportunities for integrating UAVs into 5G networks. %technologies for this type of network security solutions.
In continuation we discuss several detection and mitigation procedures to counter the principal attacks described in the previous section. %the security threats specifically eavesdropping and sniffing in UAV-cellular integration network. 
 
\begin{table*}[ht]
\centering
\caption{5G security requirements and opportunities for UAVs}
\vspace{-2mm}
\label{tab:my-table2}
%\resizebox{0.85\textwidth}{!}{%
{
%\begin{tabular}{|c|c|c|}
\begin{tabular}{|p{2cm}|p{3.2cm}|p{10.8cm}|}
\hline
%\begin{tabular}[c]{@{}c@{}}
\textbf{Mechanism}%\end{tabular} 
& \textbf{Enabling Technology} & \textbf{Description} 
\\ \hline
%\begin{tabular}[c]{@{}c@{}}
Authentication and Key Agreement %(EAP-AKA)%\end{tabular} 
&
%\begin{tabular}[c]{@{}c@{}}
Public Key Infrastructure and certification authority%\end{tabular} 
&
%\begin{tabular}[c]{@{}c@{}}
Mutual authentication and encryption must be supported at both ends of the communication link for A2A, A2G and G2A. Certificates used in A2A need to be issued by a central authority and be verifiable by the nodes. %\\ and will be used for mutual authentication and subsequent\\ service security and encryption procedures.
%\end{tabular} 
\\ \hline
Distributed control & Blockchain & %\begin{tabular}[c]{@{}c@{}}
Blockchain with intrusion detection systems can be used for detecting UAV attacks and false transactions between UAVs and macro base stations.%\end{tabular}
\\ \hline
Relay node selection & %\begin{tabular}[c]{@{}c@{}}
Relaying
 %\end{tabular} 
& %\begin{tabular}[c]{@{}c@{}} 
UAVs can relay transmitted packets between ground users and ground users can rely packets between UAVs to avoid eavesdroppers.
%\end{tabular} 
\\ \hline
Beamforming & %\begin{tabular}[c]{@{}c@{}}
Multi-antenna system %\end{tabular} 
& %\begin{tabular}[c]{@{}c@{}}
UAV-cellular network security can be boosted by taking the advantage of directional and narrow beams of 5G.%\end{tabular} 
\\ \hline
Mobility management & %\begin{tabular}[c]{@{}c@{}}
%Trajectory control
Maneuverability %\end{tabular} 
& %\begin{tabular}[c]{@{}c@{}}
UAVs have additional degrees of freedom for movement and their location, trajectory and maneuverability can be leveraged by the network to increase the secrecy rate.
%\end{tabular} 
\\ \hline
Resources allocation &% Power control & %\begin{tabular}[c]{@{}c@{}}
Control signaling
 %\end{tabular} 
& %\begin{tabular}[c]{@{}c@{}}
Resource selection and power control %Adjusting the power levels of wireless links 
can enhance the ability to mitigate sniffers from capturing exchanged information between authenticated nodes.
%\end{tabular} 
\\ \hline
%Resources allocation and 
Network segmentation & %\begin{tabular}[c]{@{}c@{}}
 %\end{tabular} 
Network slicing and orchestration
&  %\begin{tabular}[c]{@{}c@{}}
Network operators can define and manage network slices specifically designed for UAS communications and networking to follow stricter security policies, implement stronger security mechanisms, or employ a more dynamic mapping of virtual network functions to physical resource.% and have the ability to limit and contain the eavesdropper nodes can be used to define a special network slices for UAVs connections.
%\end{tabular} 
\\ \hline
\end{tabular}%
}
\end{table*}

% \begin{table}[hb]
% \centering
% \caption{5G security solutions for UAVs }
% \label{tab:my-table2}
% \resizebox{0.49\textwidth}{!}{%
% \begin{tabular}{|c|c|}
% \hline
% \begin{tabular}[c]{@{}c@{}}5G security\\ solutions\end{tabular}                       & Description                                                                                                                                                                                                  \\ \hline
% \begin{tabular}[c]{@{}c@{}}Authentication and \\ Key Agreement (EAP-AKA)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Must be supported by both ends of the communication links \\ and will be used for mutual authentication and subsequent\\ service security and encryption procedures.\end{tabular} \\ \hline
% Blockchain-based UAV                                                                  & \begin{tabular}[c]{@{}c@{}}By integrating the blockchain with intrusion detection \\ system (IDS) for detecting UAVs attacks and false \\ transactions between UAVs in macro eNB (5G).\end{tabular}          \\ \hline
% 5G mmWave                                                                             & \begin{tabular}[c]{@{}c@{}}UAVs-Cellualar network security can be boosted by taking \\ the advantage of directional and narrow beams of 5G\\ mmWave.\end{tabular}                                            \\ \hline
% \end{tabular}%
% }
% \end{table}

\subsection{Detection}

\subsubsection{Network Data Analytics}
One effective way of optimizing cellular network performance is collecting and analyzing performance measurement (PM) counters and key performance indicators (KPIs) for diffent part of the network.
Modern base stations capture hundreds of these and store and process the huge amount of data that is collected over weeks or months.
Research has shown that RF attacks on LTE networks can leverage these PM counters and KPIs to identify sophisticated signaling attacks~\cite{MarVTC17}. %The authors use classification techniques to distinguish normal operation from anomalies and distinguish between different anomalies.

% \subsubsection{Spectrum Sensing}
% ...

% \hl{[Vuk]}

% 5G will use many spectrum bands and leverage unlicensed and shared spectrum...


\subsubsection{Protocol Procedures}
%Apart from making control and data signaling more robust, 
Special control channels, packets, or frames can be introduced and scheduled to facilitate the detection of wireless attacks. Examples include blank subframes, reporting of transmit power levels and received control information, and exchanges of concealed credentials. The UAS-UEs should monitor and evaluate the legitimacy of advertised networks and network identities--just like regular UEs should do to avoid control channel spoofing from fake base stations~\cite{LabCM2017}. Leveraging UAS dynamics, the received signals/messages can be checked against location, trajectories and prior observations, or preloaded information specific to the UAS mission.

%\hl{[VUK to include more based on 5G security specs and link to table]}

\subsubsection{Intrusion Detection System (IDS)}
Reference~\cite{1} uses an IDS to detect and identify malicious UAVs in an aerial ad hoc network for minimizing the false positive and negative rates of the system. %~\cite{1}.  %by utilizing estimation algorithm based on belief approach \cite{1}. 
A two-step IDS is introduced in~\cite{2} to detect the attackers in  UAV communications systems. It consists of a traffic characterization module that is based on spectral analysis and a robust controller to reconstruct the attack.

\subsection{Mitigation}

\subsubsection{Relay Node Selection}
The 5G network architecture is designed to connect and link a wide range of devices and enable vertical applications (e.g. the smart grid, smart city, enhanced C-V2X and massive IoT) while providing higher system scalability and flexibility. Such diversity of available devices and network edge nodes can be leveraged for advanced relaying, %(mobile or fixed), 
including full-duplex, mobile, cognitive and Device-to-Device (D2D) relaying. The security of all nodes in the system can be increased by taking advantage of the heterogeneous nature of 5G relays. %as far as possible. 
Moreover, relay selection can be carefully optimized to secure specific links. %as part of the relay selection process. 
In this paper we will show how %more robustness to the security
the information secrecy can be improved when using selected UAVs %as relays approach 
for relaying the messages between two ground users with the existence of an eavesdropper. Moreover, we will discuss a new perspective of UAV relaying %as relays between users by
where we take advantage of UAV height adjustments to maximize the secrecy rate. The results are presented in Section~\ref{sec:results}-A. %This schemes has shown an improvement results with respect to the secrecy rate which will be mentioned in Section \ref{sec:results}-A. 

\subsubsection{Beamforming} 
5G will use massive full-dimension multiple-input multiple-output (MIMO) to enable 3D beamforming. %be equipped by advanced techniques for transmit and receive packets over massive antenna systems. %such as massive MIMO. %and beamforming. 
Furthermore, 5G will operate in microwave and millimeter wave (mmWave) bands. %for locating of objects and providing the range, velocity and angle of these objects. 
Researchers~\cite{6} have shown that increasing directionality and reducing the beam width %using a more concentrated array gain 
is useful for enhancing %mmWave 
the network secrecy efficiency. The excessive degrees of freedom of future 5G base stations can be effectively leveraged to protect UAV communications links. %, the secrecy can be increased between UAVs an Using such techniques for UAV-to-UAV links will be more efficient and applicable due to high mobility pattern provided by the natural features of UAV flying environment.  


\subsubsection{Resource Allocation}
Resources in next generation wireless communications networks can be managed in such as way to effectively improve the system's secrecy capacity. % of the system. 
The secrecy capacity is the result of the distinguishing between the communication channels of the eavesdropper and legitimate users taken into consideration the channel capacity. The perfect secrecy capacity is defined as the difference in capacity between those two channels, where the eavesdropper channel have been degraded more than the legitimate channel. %Next, we are going to give a brief description of how can different 5G resource allocation schemes can be used to enhance the security of UAS integration with 5G.

Another technique %to use security-aware resource allocation 
for improving the overall system security is power control. %Power control aims to adjust the transmission power levels of the nodes to stop eavesdropper from capturing the transmitted packets between authenticated nodes. 
The authors of~\cite{5} introduce a Stackelberg game framework for optimizing the achieved rate of cellular users and the secrecy rate of D2D users in 5G based on power and admission control. %and channel access of single. 
Power control combined with other mechanisms described here can be critical for securing UAVs communications in 5G.% cellular network specifications. 

\subsubsection{{Network Slicing}}%Scheduling
Network slicing is one of the pillars of 5G for enhancing the network reconfigurability and scalability, while providing resource isolation. The network operator has more dynamic control over each slice to make it easier to configure and change each one individually according to the actual deployment contexts and needs. %(e.g. available bandwidth, maximum density and transport protocols). 
This can be useful for security, as it allows to %from one point of view, where you 
divide a diverse and wide network into smaller segments where each segment can define the policy, context and mechanisms for security. Also, it facilitates to provide more or fewer security features on %context then you can provide specific security to
the different slices. On the other hand, if an eavesdropper has sufficient information about a network slice--such as, what it is used for and who uses it--then an effective attack can be launched. %may developed based on this data. 
This feature can be used for enhancing A2G and A2A links, using more demanding security policies for those slices based on the particularities of these links. % or limit the access based on the power level.
%scheduling policies   %virtualized schedulers 

% \paragraph{Resource Allocation}
% Another technique to use security-aware resource allocation for improving the overall system security. %is power control. %Power control aims to adjust the transmission power levels of the nodes to stop eavesdropper from capturing the transmitted packets between authenticated nodes. 
% The authors of~\cite{5} introduce a Stackelberg game framework for optimizing the achieved rate of cellular users and the secrecy rate of D2D users in 5G based on power and admission control. %and channel access of single. 
% Power control combined with other mechanisms described here can be critical for securing UAVs communications in 5G.% cellular network specifications. 

%\paragraph{Cell association}

%If am attacker can be located, users can be associated to other cells (macro, micro, femto) or operate in V2V mode, or use the advance communications technology to avoid the attacker and the affected cell...
%...



\subsubsection{Protocol Hardening} The 5G RAN can be protected in different ways, which can be combined. As the first need for hardening 5G signaling is proper and consistent encryption of signals and messages, for both ad hoc (UAV-to-UAV) and regular cellular network operation (A2G, G2A) modes. Agile signaling and higher order signal processing can give additional gains. Agile signaling, where the control and data channel are not fixed and can be mapped to different physical resources and scheduled (with additional redundancy) as needed to create unique signatures that can aid in the demodulation under severe interference, or can simply make it less interesting for attackers to implement protocol-aware RF attacks.


%\subsubsection{Artificial Noise} ....

%[Lingjia and Bodong?]



==> include/research.tex <==
%C-V2X Mode 4 is an ad-hoc communication mode using the PC5 air interface between UEs. In this mode, the peers are not known a priory and change dynamically because of the different trajectories of vehicles. Since infrastructure is not involved in this mode, standard LTE security mechanisms cannot be applied. 3GPP does not address the establishment of adhoc security associations in R14.
Cellular infrastructure-based and ad-hoc networking have different requirements and constraints, but security needs to be implicit to both. 
5G will enable both types of communications and 3D mobility through UAVs. It is essential to analyze and identify the key vulnerabilities and effective security mechanisms when introducing a new communications mode. %, and propose and demonstrate mechanisms to harden it. 
Research in the following areas can be leveraged to increase the security of 5G for servicing UAVs and ensuring their reliable operation:

\begin{itemize}
    \item \textbf{Physical layer techniques.} Use and leverage the diversity of the channel as well as interference mitigation techniques. Embed signatures or other unique identifiers in messages to identify legitimate UEs and legitimate messages. %5G will need to leverage PHY layer security, which can relieve implementing computing intensive encryption and other security mechanisms where not practical.
    
    \item \textbf{Cross-layer techniques.} Modify scheduling, congestion control and other 5G procedures to improve their robustness and increase the awareness of potential threats (e.g., scheduling messages for the purpose of enhancing distributed security awareness).
    
    \item \textbf{Edge and Cloud computing.} Use the Cloud to assist in determining fake transmitters and leverage edge computing to reduce latency and network congestion. Security mechanisms need to be implicitly in place since 5G VNFs will be sharing physical platforms where they run with other applications.
    
    %\item \textbf{Network-aided procedures.} Have the network periodically notify UEs of legitimate UEs in the area using C-V2X or parallel communications protocols, such as regular LTE.
    
    %\item \textbf{Radio environment map (REM).} Have UEs built their REMs, where processed RF spectrum activity and the information exchanged among UEs is stored and contrasted to identify anomalies.
    
    \item \textbf{Spectrum sharing security.} The aerial UEs and network nodes can regularly sense RF environments, process, and forward it for centralized or distributed RF anomaly detection. It is critical that the spectrum access system database %for shared spectrum access 
    is secure and monitored.
    
    \item \textbf{Data collection and analyses.} Data gathered from experiments or during operation needs to be processed and made available for inferring 5G operational contexts and classifying known and unknown anomalies. %can ML can be effectively employed to analyze huge amounts of data and classify it. When either the normal behavior is known or the attacks, ML tools can be trained to distinguish between normal and abnormal activity.
    
    \item \textbf{Sensor fusion.} Physical attributes, past messages, environmental contexts, etc. and information coming from multiple sensors can be used to validate messages, weigh decisions and dynamically update node and information thrust metrics. %Message content for consistency 
\end{itemize}

%Research has shown that combining multiple sources of data can help identifying and overcoming a threat. %An example of this is jointly processing several of the widely used performance measurement counters and key performance indicators in cellular networks to identify a specific source of interference. 

% The following tools can be leveraged for accelerating research, testing, and standardization:

% \begin{itemize}
%     \item Software-defined radios and open-source software,
%     \item Laboratory and field experiments, providing data for researchers to use, 
%     \item Crowdsourcing, allowing distributed development and testing as well as contributions to specifications,
%     \item Specifications with more dynamic contributions,
%     \item Regular firmware and software updates and secure software downloads and installations for radios and wireless networking equipment and at a rate comparable to IT systems, 
%     \item Use of virtualization technology to enable dynamic network reconfiguration and security as a service. 

% \end{itemize}




One of the main challenges is the real-time nature of the data and the limited resources (time, RF bandwidth, and processing power) that are available. Moreover, the interference or attack may change. Therefore, one solution will not fit all cases and a single approach may result ineffective. Instead, several techniques should be combined and used in concert. For example, the UAS can do some local processing and combine it with data processed at the network edge or Cloud, or the data provided by the network. 

